MinUn: Accurate ML Inference on Microcontrollers

Running machine learning inference on tiny devices, known as TinyML, is an emerging research area. This task requires generating inference code that uses memory frugally, a task that standard ML frameworks are ill-suited for. A deployment framework for TinyML must be a) parametric in the number representation to take advantage of the emerging representations like posits, b) carefully assign high-precision to a few tensors so that most tensors can be kept in low-precision while still maintaining model accuracy, and c) avoid memory fragmentation. We describe MinUn, the first TinyML framework that holistically addresses these issues to generate efficient code for ARM microcontrollers (e.g., Arduino Uno, Due and STM32H747) that outperforms the prior TinyML frameworks.

==> sections/10-acknowledgements.tex <==
\begin{acks}                            %% acks environment is optional
                                        %% contents suppressed with 'anonymous'
  %% Commands \grantsponsor{<sponsorID>}{<name>}{<url>} and
  %% \grantnum[<url>]{<sponsorID>}{<number>} should be used to
  %% acknowledge financial support and will be used by metadata
  %% extraction tools.
%   This material is based upon work supported by the
%   \grantsponsor{GS100000001}{National Science
%     Foundation}{http://dx.doi.org/10.13039/100000001} under Grant
%   No.~\grantnum{GS100000001}{nnnnnnn} and Grant
%   No.~\grantnum{GS100000001}{mmmmmmm}.  Any opinions, findings, and
%   conclusions or recommendations expressed in this material are those
%   of the author and do not necessarily reflect the views of the
%   National Science Foundation.
We would like to thank Oindrila Saha, Shubham Ugare, Prateek Jain and Harsha Vardhan Simhadri for their useful insights and discussions on this work.
\end{acks}

==> tables/fixed_point_latency.tex <==
\begin{table*}
\footnotesize
\caption{Latency values of \fastgrnn, \protonn, \bonsai and \rnnpool models for \previoustoolfixed and \toolfixed generated codes. Latency values are in seconds. For classification-based models, the number of classes follow the dataset name.}
\vspace{3mm}
\centering
\begin{tabular}{c|c|c}
\multicolumn{1}{c}{\textbf{Model \&}} & \multicolumn{1}{|c}{\textbf{\previoustoolfixed}} &
\multicolumn{1}{|c}{\textbf{\toolfixed}} \\ 
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{|c}{\textbf{Latency}} & \multicolumn{1}{|c}{\textbf{Latency}}\\
\toprule
\multicolumn{1}{c|}{\textbf{\fastgrnn}} & &\\
DSA-19 & 1.964 & 2.047\\
WAKEWORD-2 & 1.167 & 1.124\\
GOOGLE-12 & 2.645 & 2.718\\
GOOGLE-30 & 3.043 & 3.060\\
HAR-2 & 2.690 & 2.633\\
HAR-6 & 3.201 & 2.990\\
USPS-10 & 1.094 & 1.172\\
MNIST-10 & 0.901 & 0.903\\
INDUSTRIAL-72 & 0.092 & 0.092\\
\midrule
\multicolumn{1}{c|}{\textbf{\protonn}} & &\\
CIFAR-2 & 0.003 & 0.004\\
CR-2 & 0.006 & 0.007\\
CR-62 & 0.008 & 0.007\\
CURET-61 & 0.007 & 0.008\\
LETTER-26 & 0.010 & 0.010\\
MNIST-2 & 0.004 & 0.004\\
MNIST-10 & 0.004 & 0.004\\
USPS-2 & 0.003 & 0.003\\
USPS-10 & 0.004 & 0.005\\
WARD-2 & 0.004 & 0.005\\
\midrule
\multicolumn{1}{c|}{\textbf{\bonsai}} & &\\
CIFAR-2 & 0.002 & 0.002\\
CR-2 & 0.002 & 0.002\\
CR-62 & 0.010 & 0.010\\
CURET-61 & 0.013 & 0.015\\
LETTER-26 & 0.004 & 0.005\\
MNIST-2 & 0.002 & 0.003\\
MNIST-10 & 0.004 & 0.005\\
USPS-2 & 0.002 & 0.002\\
USPS-10 & 0.003 & 0.003\\
WARD-2 & 0.003 & 0.003\\
\midrule
\multicolumn{1}{c|}{\textbf{\rnnpool}} & &\\
FACE-A & 16.661 & 16.864\\
FACE-B & 7.880 & 7.942\\
FACE-C & 9.440 & 9.140\\
\bottomrule
\end{tabular}
\label{tab:fixedPointLatency}
\end{table*}
